MICADO PSF-Reconstruction work package description

The point spread function reconstruction (PSF-R) capability is a deliverable of the MICADO@ESO-ELT project. The PSF-R team works on the implementation of the instrument software devoted to reconstruct the point spread function (PSF), independently of the science data, using adaptive optics (AO) telemetry data, both for Single Conjugate (SCAO) and Multi-Conjugate Adaptive Optics (MCAO) mode of the MICADO camera and spectrograph. The PSF-R application will provide reconstructed PSFs through an archive querying system to restore the telemetry data synchronous to each science frame that MICADO will generate. Eventually, the PSF-R software will produce the output according to user specifications. The PSF-R service will support the state-of-the-art scientific analysis of the MICADO imaging and spectroscopic data.

==> text_spie.tex <==
MICADO is the Multi-AO Imaging Camera for Deep Observations. It will
equip the ESO ELT with a first light capability for diffraction limited
imaging and long-slit spectroscopy at near-infrared wavelengths.
MICADO is a workhorse instrument for the E-ELT. While its primary
focus is AO-assisted imaging, it provides a high level of flexibility
for modes that are not necessarily offered by other E-ELT instruments,
and that may lead to observations with a major scientific impact.

The instrument will work with a multi-conjugate laser guide star
adaptive optics system (MCAO, developed by the MAORY consortium) as
well as a single-conjugate natural guide star adaptive optics system
(SCAO, developed jointly by the MICADO and MAORY consortia). It will
interface to the MAORY warm optical relay that re-images the telescope
focus. In this configuration, both MCAO and SCAO are available. If
required for an initial phase, MICADO will also be able to operate
with just the SCAO system in a ``stand-alone'' mode, using a simpler
optical relay that interfaces directly to the telescope. MICADO has
four observing modes producing data: Standard Imaging, Astrometric
Imaging, High-contrast Imaging, and Spectroscopy.

Each observing mode can optionally be operated in a configuration that
gathers the data (WFS images and telemetry) required for PSF
reconstruction. [RD23] provides a detailed description of the Calibration
Plan for the four Observing Modes and the PSF Reconstruction.

PSF-R tools are not foreseen for the High-contrast imaging mode,
because this mode focuses instead on canceling the PSF using peculiar
observational and instrumental techniques. Moreover, the PSF-R
Applications will not work for the seeing enhancer and seeing limited
(No-AO) modes described in [AD4]. Non-sidereal imaging mode data will
not be suitable for PSF-R application if a spatially resolved moving
target will be used as AO guide star for WFS.

The Data Reduction Library Design document for PSF-R Application
provides the detailed design of the software recipes required for the
analysis of Adaptive Optics data from the MICADO instrument at the
ELT. The aim of these libraries is to produce state-of-the-art
computations of the reconstructed PSF of MICADO.

PSF-R is the process to determine the PSF of a
science exposure, without using the focal plane pixel data in the
science image. The reconstructed PSF is instead estimated using (i)
pixel data and telemetry generated by the Adaptive Optics system, (ii)
information by other systems monitoring the atmosphere and (iii)
telemetry from the ELT and MICADO instrument.

The PSF-R service for the MICADO instrument at the ELT
will provide a service to the following observing modes:
\begin{itemize}
\item
Standard imaging
\item
Astrometric imaging
\item
Spectroscopy.
\end{itemize}

PSF-R is not foreseen for the High-contrast imaging mode,
because this mode focuses instead on canceling the PSF using observational
and instrumental techniques.

PSF-R is a service that complements, but is not part of,
the data processing pipeline. It is a tool that assists data analysis
rather than data reduction. To reconstruct a full 2D PSF (or even
parameters describing it) is a complex procedure that requires careful
calibration. To date, no ground-based observatory offers PSF
reconstruction as a facility tool for adaptive optics
observations. This is what is planned for MICADO, but it has to be
done as a collaborative development involving the ELT and MAORY as
well as MICADO, since all these systems contribute to the final
measured PSF, and they all have a role in saving and archiving the
necessary data. One of the requirements for PSF reconstruction is to
match the irregularities in the PSF and
variations across the field of view seen in real observations.

The accuracy of the reconstructed PSF in reproducing the observed PSF
of a science image is driven by the Scientific requirements of MICADO.
The goals of the PSF-R service is to
provide reconstructed PSFs with defined metrics (Strehl ratio,
Encircled Energy, FWHM, Ellipticity, etc.) within the reference values
summarized in Table XX. The quoted accuracies have been
derived by analytic calculations and they should be refined with
simulations carried out by the MICADO Science Team and by the Work
Package Scientific Evaluation Simulations of PSF-R.

